Improving Compositional Generalization with Latent Structure and Data Augmentation

Generic unstructured neural networks have been shown to struggle on out-of-distribution compositional generalization. Compositional data augmentation via example recombination has transferred some prior knowledge about compositionality to such black-box neural models for several semantic parsing tasks, but this often required task-specific engineering or provided limited gains. We present a more powerful data recombination method using a model called Compositional Structure Learner (CSL). CSL is a generative model with a quasi-synchronous context-free grammar backbone, which we induce from the training data. We sample recombined examples from CSL and add them to the fine-tuning data of a pre-trained sequence-to-sequence model (T5). This procedure effectively transfers most of CSL's compositional bias to T5 for diagnostic tasks, and results in a model even stronger than a T5-CSL ensemble on two real world compositional generalization tasks. This results in new state-of-the-art performance for these challenging semantic parsing tasks requiring generalization to both natural language variation and novel compositions of elements.

==> backup/0_abstract.tex <==
\tl{What about the abstract wouldn't also describe Shaw et al 2021?} Popular neural network architectures such as sequence-to-sequence models have been shown to struggle on out-of-distribution compositional generalization, where the model is presented with novel combinations of the elements observed during training. Specialized approaches with discrete latent structure have demonstrated significant improvements on synthetic evaluations of compositional generalization, but such approaches are often outperformed by pre-trained sequence-to-sequence models such as T5 on non-synthetic tasks. We present a learning algorithm and generative model based on a quasi-synchronous context free grammar, which we refer to as CSL. We also present a method for combining the relative strengths of CSL and T5, sampling new synthetic examples from CSL to use for training T5. Our method effectively solves several synthetic evaluations of compositional generalization, and outperforms the state-of-the-art across multiple evaluations of compositional generalization on non-synthetic tasks.

==> backup/1_introduction.tex <==
\section{Introduction}\ps{Todo... revise to focus more on data augmentation, less rehash ACL paper narrative}

\include{figures/method_diagram_v2}
\eat{
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/method_diagram.pdf}
    \caption{Todo... And redo the figure in tikz...Would an example from non-synthetic data fit as well? A: How about COGS? GeoQuery and SMCalFlow would be too verbose I think.}
    \label{fig:method_diagram}
\end{figure}
}

Compositional generalization refers to the ability to generalize to novel combinations of previously observed \emph{atoms}\footnote{Also commonly referred to as \emph{elements} or \emph{concepts}.}. For example, we may assess a model's ability to interpret the instruction ``jump twice'', when ``jump'' and ``twice'' were each observed separately during training but were never combined with each other~\cite{lake2018generalization}.

Evaluations for compositional generalization consist of both synthetic and non-synthetic datasets, where natural language inputs are generated by programs or humans, respectively. Synthetic evaluations such as SCAN~\cite{lake2018generalization}, COGS~\cite{kim-linzen-2020-cogs}, and CFQ~\cite{keysers2019measuring} enable controlled and precise evaluations of compositional generalization. However, the language used is generally less realistic and more tightly controlled than those of non-synthetic datasets where utterances are collected from humans. Compositional splits of non-synthetic datasets, such as template~\cite{finegan2018improving}, TMCD~\cite{keysers2019measuring,shaw2021compositional}, and cross-domain~\cite{yin2021compositional} splits, therefore add the further challenge of handling natural language variation in addition to compositional generalization. A central and unsolved challenge is to develop an approach that can excel across a diverse set of evaluations covering both compositional generalization and natural language variation~\cite{shaw2021compositional}.

Specialized architectures with discrete latent structure~\cite{chen2020compositional,liu2020compositional,nye2020learning,herzig2020span,shaw2021compositional} have made the largest gains on synthetic evaluations, effectively solving SCAN and achieving high accuracy on other evaluations, although commonly with some degree of task-specific engineering. Regardless, such specialized architectures, on their own, are commonly \fs{add a few refs to support this}outperformed on non-synthetic evaluations by general purpose pre-trained models such as T5, which excel at handling natural language variation and require fewer syntactic assumptions.

% Several types of approaches have been proposed to improve compositional generalization, including new or modified architectures, data augmentation, meta-learning, and intermediate representations. Of these, several specialized architectures have been proposed that represent discrete latent structure in the mapping from inputs to outputs. In many cases, such latent structures are similar to the derivations given by traditional grammar formalisms such as Synchronous (SCFGs) and Quasi-Synchronous Context Free Grammars (QCFGs). Such formalisms effectively decompose the data generating process into a chain of rule applications, enabling rules to be flexibly recombined. These architectures have made the largest improvements on synthetic evaluations, effectively solving SCAN~\cite{} and achieving high accuracy on CFQ and COGS~\cite{}, although commonly with some degree of task-specific engineering. Regardless, as of yet, none of these specialized architectures are, on their own, competitive with general purpose pre-trained sequence-to-sequence models such as T5 on standard splits of non-synthetic tasks, limiting their utility.  It remains an open challenge to develop models that excel at compositional generalization across a diverse set of tasks and evaluations without sacrificing in-distribution performance relative to models such as T5~\cite{shaw2021compositional}. \linlu{This seems to directly jump from evaluating compositional generalization on synthetic datasets to in-distribution on non-synthetic datasets, but does not mention performance on compositional splits? Although we probably can't say specialized models always perform worse on non-synthetic tasks compared to T5 (length split might be a counter-example).}

Given their different strengths and weaknesses, it is compelling to try to combine the strong capacity for compositional generalization of such specialized models with the greater flexibility and ability to handle natural language variation of general purpose pre-trained models such as T5. 
%\linlu{does the flexible capabilities refer to handle language variation? from above, it seems to be strong in-distribution performance but I don't think we build connection between these? IMO it's not very clear here what exactly are the strengths and weaknesses of these two types of models. Will bring Figure~\ref{fig:quadrant_figures} up help illustrate this better?}
% Pete - is it clearer now? T5 = fewer syntactic assumptions, better handle natural language variation.
Such ambitions are not new. Notably, in one of the first papers applying sequence-to-sequence models to semantic parsing, \citet{jia2016data} introduce a method for data augmentation using synchronous grammars. The authors eloquently observe that \emph{``language is a blend of crisp regularities and soft relationships''}, and note that sequence-to-sequence models \emph{``excel at modeling soft phenomena''}\ps{I like these quotes because they have served as partial inspiration -- but maybe move to footnotes?} while grammars can be used to infuse an understanding of crisp structure. More recently, GECA~\cite{andreas-2020-good} has provided a more general data-augmentation algorithm, and achieved improvements on several evaluations of compositional generalization. However, such approaches are limited in the types of recombinations that can be generated for a given dataset, and have only demonstrated modest gains on \fs{can we strengthen by stating most gains are still on synthetic ones?}some evaluations.

% As an alternative method to combine discrete structure with sequence-to-sequence models, \citet{shaw2021compositional} propose a method which learns a latent variable parsing model based on an induced grammar, and falls back to T5 for examples that cannot be derived by the induced grammar. While this delivers strong performance across a diverse set of evaluations, such an approach can only offer limited improvements when the underlying grammar cannot derive all of the inputs in the evaluation set. However, one important observation from this work is that despite the apparent difficulty of developing specialized architectures that compete head-to-head with models like T5, specialized grammar-based models can outperform T5 over a specific subset of examples: out-of-distribution examples that can be derived by the induced grammar.

\eat{
In this work, inspired by this observation, we propose a new method for compositional generalization. First, we learn a generative latent variable model based on a grammar induced from the training data. We refer to this model as CSL, for Compositional Structure Learner. Then, we use CSL to sample additional training data, which we use as additional training data for T5. Our method enables new types of recombinations of the training data that are not supported by existing approaches such as GECA, while maintaining sufficiently high quality for the synthetic data. Additionally, our method outperforms an ensemble of CSL and T5 similar to that of ~\citet{shaw2021compositional}, as data augmentation enables improved performance even on out-of-distribution examples that cannot be derived by the induced grammar.}

%are not \fs{what does "directly" mean here? It is fairly intuitive to think sampled data not directly observed in the training data adds value. But this claim is not referring to that. will come back to this late after the whole paper reading.} directly derivable in the induced grammar. 
% Pete - "directly" should be removed, I think. Is it clearer?

\kt{I drafted proposed alternative framing of the work to reduce the claim that this is an entirely new approach and to focus on comparisons and learnings while also mentioning the resulting SOTA performance.}
% In this work, inspired by this observation, we study the
In this work we study the effectiveness of compositional data augmentation using an automatically induced latent synchronous context free grammar similar to that of \citet{shaw2021compositional}, where examples sampled from the grammar-based model are used to augment the training data for a ``black-box'' sequence-to-sequence model such as T5. We compare the value of the induced grammar and model (termed CSL for \textbf{C}ompositional \textbf{S}tructure \textbf{L}earner in this work) when used to form a hybrid with T5 as in NQG-T5, versus when used to generate additional training data for T5. We show that CSL is more effective for data augmentation than for model combination on non-synthetic data, and that for synthetic data combination is more effective but generated training data helps transfer most of CSL's task knowledge to T5, leading to a black-box sequence to sequence model approaching 100\% performance on all splits of the synthetic SCAN task.

CSL is more powerful for data augmentation compared to GECA (hopefully we have specific analysis or insights on that), and is also more generally applicable in comparison to the task-specific grammar induction procedure of the related SCFG-based approach of \newcite{jia2016data} (can we say something more specific here).

Unlike prior approaches, we also explore a set of models based on an SCFG backbone, which differ in their independence assumptions (context-free versus varying extent of context dependence). They provide varying trade-offs between being able to extrapolate to unseen combinations of elements versus generating valid sequences only. \kt{If we want to claim this, should report on the effect of the number of clusters.} 

We analyze the relative performance of the ensemble versus augmentation approach on different slices of the evaluation data to understand the source of the differences.  

Our method effectively solves several synthetic evaluations: SCAN, CFQ, and COGS.\ps{Edit this -- CFQ will not be solved.} Our method also outperforms the state-of-the-art across several compositional splits of the non-synthetic datasets GeoQuery and SMCalFlow-CS~\cite{yin2021compositional}. We also propose an alternative setting, where we assume the availability of some unlabeled data from the target distribution during training, and demonstrate that this can be leveraged to further improve performance.



==> backup/3_method_old.tex <==
\section{Proposed Method}
\label{sMethod}

As shown in Figure~\ref{fig:method_diagram}, our method consists of two stage. First, we describe our generative model, CSL, and how it is induced from the training data in \S\ref{sMethodModel}. Second, we discuss sampling synthetic data from our generative model and using it to train pre-trained sequence-to-sequence \S\ref{sMethodAugment}.

The key idea behind our method is to augment training with synthetic ones sampled from probabilistic generative models learned from the training data. In particular, those samples introduce novel combinations of primitives that are not observed in the training data. As such, the difference between the training and the testing distributions is reduced. Formally, in the notations introduced in the previous section, the empirical distribution of $x$ in the training data $\mathcal{D}_{\text{train}}$ captures only a subset of its domain $\mathcal{X}$ such that   the risk on the test distribution $\mathbb{E}_{p_t(x)p(y|x)} \ell(x,y)$ cannot be consistently estimated from the training distribution $p_s(x)$\footnote{More precisely, the importance weight $p_t(x)/p_s(x)$ is unbounded, thus  cannot be used for correcting covariate shift~\cite{xxx}.}.

We describe learning the generative model in \S\ref{sQCFG}. The data augmentation procedure and training T5 (or any other sequence-to-sequence models) are fairly straightforward and are briefly summarized in \S\ref{sMethodDetails}.


\subsection{Learning Generative Model}
\label{sMethodModel}

For the tasks investigated in this paper,\tl{Say a little bit about those tasks before this? At least that they're semantic parsing} we assume the training data $\mathcal{D}_{\text{train}}$ consists of pairs of input and output strings.  The data is generated by sampling a grammar's rules.\kt{Isn't this how the original training data is generated for synthetic datasets only?} Our goal is to discover the grammar and the  probabilities associated with those rules. 

\paragraph{Grammar Formalism} \ps{copied from ACL paper, need to rewrite.}We assume the grammar is an instance of Quasi-Synchronous Context Free Grammars (QCFGs). QCFGs generalize Synchronous Context-Free Grammars (SCFGs), which have been used to model the hierarchical mapping between pairs of strings in areas such as compiler theory~\cite{aho1972theory} and natural language processing. Informally, SCFGs can be viewed as an extension of Context-Free Grammars (CFGs) that \emph{synchronously} generate strings in both a source and target language. We write SCFG rules as:
$$ S \rightarrow \langle \alpha,\beta \rangle $$
Where $S$ is a non-terminal symbol, and $\alpha$ and $\beta$ are strings of non-terminal and terminal symbols. An SCFG rule can be viewed as two CFG rules, $S \rightarrow \alpha$ and $S \rightarrow \beta$ with a pairing between the occurrences of non-terminal symbols in $\alpha$ and $\beta$. This pairing is indicated by assigning each non-terminal in $\alpha$ and $\beta$ an index $\in \mathbb{N}$. Non-terminals sharing the same index are called \emph{linked}. Following convention, we denote the index for a non-terminal using a boxed subscript, e.g. $NT_{\boxnum{1}}$. A complete SCFG derivation is a pair of parse trees, one for the source language and one for the target language. An example derivation is shown in Figure ~\ref{fig:derivation_example}.

QCFGs notably relaxes the restriction of SCFGs from one-to-one alignment between source and target \fs{Is this the right way to say it, since this paper deals with one NT?}non-terminals to one-to-many~\cite{smith2006quasi}. \linlu{I think that is the case, we just allow one NT being expanded by any indexed NT.}We restrict our grammars to have only a single nonterminal symbol, $NT$.

Each rule in a QCFG is associated with a probability to indicate how likely this rule should be expanded, given the context. \linlu{More precisely it should be each indexed nonterminals in each rule? or how likely this rule "is used to expand the parent rule"}Ideally, we would like to maximize the likelihood of the training data with respect to all possible QCFGs and their parameterizations. In this work, we use an approximate, more efficient two-step process instead. In the first step, we induce a QCFG from the training data. In the second step, we learn the parameters of a model decomposing over rule applications from the QCFG.\tl{What does "decomposing over rule applications" mean?}
%While this is quite expensive, this work simplifies with a two-step process.

\paragraph{Grammar Induction}   Our method for inducing a QCFG is based on that of \citet{shaw2021compositional}, but with several modifications. The primary purpose of the modifications is to improve the computational efficiency of the algorithm so that it can effectively scale to larger datasets and longer pairs of strings. 
% \linlu{I think this might need to be moved to under 3.1? the only thing new here is the induction objective, but this section doesn't seem to explain how this could improve computational efficiency. IMO we have two major changes help improving computational efficiency: (1) we use sampling instead of considering every rule and (optionally approximate dataset codelength by sampling as well); (2) we use generative model to avoid computing partition function)} \ps{There are several other key sub-routines that are changed as well, notably `unification_utils`. Too much to explain here. Can in appendix.} \linlu{sg}

The main idea of the grammar induction is to balance the size of the grammar with its ability to parse the training data. Similar to the inductive objective in \citet{shaw2021compositional}, we apply the principle of minimum description length (MDL) to reduce (the weighted sum of) the counts of terminal and nonterminal tokens in the grammar. To capture the ability of the grammar, \citet{shaw2021compositional} needs to count the number of derivations in the grammar--essentially the conditional probability of $p(y|x)$ which requires computing the partition function of $p(x)$. This is expensive for large datasets and long strings. Thus, we use a surrogate which measures the correlations between the input and output sides of a proposed rule $r: NT \rightarrow \langle \alpha,  \beta\rangle$, similar to that of \fs{todo?}todo:
\begin{equation}
c( r) = k_{\alpha}  \ln \hat{p}(\alpha | \beta) + k_{\beta} \ln \hat{p}(\beta | \alpha)
\end{equation}
where $\hat{p}(\alpha | \beta)$ is equal to the fraction of examples $\langle x,y \rangle \in \mathcal{D}_{train}$ where there exists some substitution of the non-terminals in $\alpha$ such that it is a substring or equal to $x$ out of the examples where there exists some substitution of the non-terminals in $\beta$ such that it is a substring or equal to $y$, and vice versa for $\hat{p}(\beta | \alpha)$.\tl{I found this paragraph hard to follow}\kt{I changed the notation a bit from $p$ to $\hat{p}$ and also added natural log symbol in the objective.}
The overall objective we minimize is thus
\begin{equation}
L(\mathcal{S}) =  k_t c_t(\mathcal{S}) + k_{nt}  c_{nt}(\mathcal{S}) +
\sum \limits_{r \in \mathcal{S}} c( r)
\end{equation}
Where $c_t(\mathcal{S})$ and $c_{nt}(\mathcal{S})$ are the counts of terminal and nonterminal tokens in $\mathcal{S}$.

To minimize, we use the greedy algorithm in  \citet{shaw2021compositional}. Details are described in the appendix.


\paragraph{Probabilistic Model} Given an induced grammar $\mathcal{S}$, we learn a model $g$ to assign probabilities to its derivations. We factorize the probability of a derivation in terms of conditional probabilities of sequentially expanding a rule from its parent.\tl{Isn't this always the case in a CFG? Each application of a rewrite rule is independent from the others?} Formally, let $r$ denote a rule, expanded from its parent rule $r_p$'s $NT_{\boxnum{i}}$ nonterminal (or a special symbol at the root of the derivation tree). We assume conditional independence and \fs{The following equation has a notation hazard as the $\theta$ is also used later to denote the neural network's outputs or parameters}factorize the probability of $z$ as
\begin{equation}
g(z) = \prod \limits_{r, r_p, i \in z} p_{\theta}(r|r_p,i)
\end{equation}
Using the example derivation from Figure ~\ref{fig:derivation_example}, for the rule application $r = \mbox{NT}  \rightarrow \langle \mbox{walk},\mbox{WALK}\rangle$, we have
\[r_p = \mbox{NT} \rightarrow \mbox{NT}_\boxnum{1} \mbox{ and } \mbox{NT}_\boxnum{2}, \mbox{NT}_\boxnum{1} \mbox{NT}_\boxnum{2},\]
and the expansion probability for that rule application is  $p(r|r_p,2)$. This non-terminal annotation with context from the tree is akin to parent annotation or other structure conditioning for probabilistic context-free grammars~\cite{johnson98,klein-manning-2003-accurate}.

To parameterize those conditional probabilities, \fs{This type should be re-texted if we have results on sweeping thru the number of types.}we propose a \fs{We probably discuss/cite Kim's latent QCFG work}latent model where we softly cluster the parent rules into a set of \emph{types} of parent rule application contexts:\tl{Can you give an intuition for what a "type" is? Also, motivate the types when you introduce them, rather than at the end of the section}
\begin{equation}
p_{\theta}(r|r_p,i) =  \sum \limits_{t \in \mathcal{T}} p_{\theta}(r|t)p_{\theta}(t|r_p,i)
\end{equation}
The two factors are then parameterized with two neural nets with softmax outputs:
\begin{align}
p_{\theta}(t|r_p,i) & = \frac{e^{\theta_{r_p,i,t}}}{\sum \limits_{t` \in \mathcal{T}} e^{\theta_{r_p,i,t`}} }\\ 
p_{\theta}(r|t) & =  \frac{e^{\theta_{t,r}}}{\sum \limits_{r` \in \mathcal{S}} e^{\theta_{t,r`}} }
\end{align}
where the $\theta$s are the outputs of the neural nets. Details of the setups of the neural nets are described in the appendix.
%\begin{equation}
% p_{\theta}(r|r_p,i) = \sum \limits_{t \in \mathcal{T}} \frac{e^{\theta_{r_p,i,t}}}{\sum \limits_{t` \in T} e^{\theta_{r_p,i,t`}} } * \frac{e^{\theta_{t,r}}}{\sum \limits_{r` \in \mathcal{S}} e^{\theta_{t,r`}} }
%\end{equation}

The model $g(z)$ is trained by maximizing the log-likelihood of $p_{\mathcal{S}, g}(x,y)$. We use a variant of the CKY algorithm to determine the set of derivations, represented as a parse forest, and use dynamic programming to efficiently sum over this set.

The number of types, $|\mathcal{T}|$ is a hyperparameter that we can use to control the capacity of the model. A smaller $|\mathcal{T}|$ may help avoid overfitting, and could potentially lead to better transfer from the source to target distribution. For example, a smaller set of types could correspond to latent syntactic categories that are shared between the source and target distributions, rather than modeling the probability of specific rule combinations that are likely to change between the source and target distributions. \linlu{Maybe we could also add some related qualitative analysis on synthetic dataset in appendix?}\kt{Analysis on synthetic data would be great.}


\paragraph{Semi-supervised learning} We can extend  to the setting when we have unlabeled data (from the target distribution). To avoid marginalizing over all possible derivations for the unlabeled data, we first use the labeled data to learn a model $g(z)$. We then use $g(z)$ to label the unlabeled data with the derivations with the highest scores. \fs{Is this correct? If not, please correct. The original text did not say anything what to do once we have noisily labeled data.}We then combine the data to derive a new grammar and a new model $g'(z)$. \linlu{I think we will only retrain the model as grammar won't change?}

%, consisting of inputs only, we can incorporate this data when training our generative model in a straightforward way. We maximize both the likelihood of $p(x,y)$ for $D_{train}$ and the marginal likelihood $p(x)$ for the unlabeled data. As the latter requires marginalizing over derivations for $x$ and all possible outputs, we approximate this by first labeling the unlabeled data with the highest scoring derivation given a generative model trained only on $D_{train}$, which can be interpreted as a {hard-EM} approach. As the induced grammar may not be able to derive all 


\paragraph{Do not know what to do yet - as we would need table of results to support the claim}Perhaps surprisingly, we found that for a given induced grammar, our simple generative model has comparable \fs{Can we refer to a table for the results or give the numbers here?} \linlu{This will be the comparsison between CSL and NQG} accuracy when used as a discriminative model for most tasks as the BERT-based model of \citet{shaw2021compositional}, despite containing far fewer parameters. As a generative model, we also avoid computing a costly partition function. While we demonstrate the effectiveness of our simple generative model, incorporating pre-trained representations within a generative model could be a promising future direction.\tl{Not sure this paragraph is necessary anywhere but if anything it should be later, not when describing the model}


\subsection{Data Augmentation} 

We synthesize data using our induced grammar $\mathcal{S}$ and the probabilistic generative model $g$.\tl{Potentially counterintuitive that you want to generalize to different distributions over derivations, but you generate the augmentation data from the same distribution as training} To generate a synthetic example $(x, y)$, we use forward sampling:  we start from the single $NT$ symbol and sample recursively from  $g$ to expand each nonterminal symbol with a rule. 

Given sequence-to-sequence models usually struggle on length extrapolation~\citep{newman2020the}, we optionally add a nonterminal bias $\delta > 0$ to softmax logits to bias towards rules with nonterminals. Namely, if a rule $NT\rightarrow \langle \alpha, \beta\rangle$ contains $NT$ in $\alpha$, then
\begin{equation}
    \theta_{t,r} \leftarrow \theta_{t,r} + \delta
\end{equation}

If a CFG $G_\mathcal{Y}$ is provided for the output language, we ensure the sampled $y$ is in $G_\mathcal{Y}$ by discarding examples for which $y$ cannot be parsed.


% The probability of sampling a rule $r$ to expand a nonterminal token $nt$ is defined as:
% $$ p_s(r|nt) = \sum \limits_{t \in \mathcal{T}} \frac{e^{\frac{\theta_{nt,t}}{\gamma}}}{\sum \limits_{t` \in T} e^{\frac{\theta_{nt,t`}}{\gamma}}} * \frac{e^{\frac{\theta_{t,r}}{\gamma} + \alpha}}{\sum \limits_{r` \in \mathcal{S}} e^{\frac{\theta_{t,r`}}{\gamma} + \alpha} }$$
% We then optionally re-label the $x$ with $y' = \max p(y|x)$ and use the $(x, y')$ as our synthetic example. This aims to deal with the ambiguity when more than one inputs can be mapped to the same output. 
\linlu{we sample from the intersection of QCFG and Gy might be more related to what we're doing.}

\subsection{Sequence-to-Sequence Model} 

We \fs{We do not have much to say here, right?}fine-tune T5 on the union of the original training data and the synthesized data.\kt{Are any weights used on the synthetic examples?}





==> backup/4_experiments_old.tex <==
\section{Experiments and Analysis}

% We divide our experiments into three sections. First, we study the effectiveness of our approach on synthetic evaluations of compositional generalization. 

\subsection{Synthetic Evaluations}
\label{sec:synthetic-evals}

We first evaluate our approach on synthetic benchmarks designed for controlled assessments of compositional generalization.
In these benchmarks, subsidiary challenges such as language variation are minimized, and the information needed to parse test sentences are guaranteed to appear in training data.\kt{It may be hard to guarantee all information needed (by which algorithm? or humans) appears in the training set.}
%Such evaluations allow for controlled assessments, and each has been constructed to ensure that every \emph{element} that appears in the evaluation set appears in the training set, for some definition of \emph{element}.

\subsubsection{Datasets}
%We selected three popular synthetic datasets for evaluating compositional generalization:

\paragraph{SCAN}
The SCAN dataset contains navigation commands paired with action sequences. We consider three compositional data splits from \citet{lake2018generalization}: the \emph{jump} and \emph{turn left} splits (where a new primitive is used in novel combinations), and the \emph{length} split (where test sequences are longer than training ones).
We also consider the \emph{MCD} split from \citet{keysers2019measuring} created by making the distributions of compositional structures in training and test data as divergent as possible.

\paragraph{CFQ}
The CFQ dataset \cite{keysers2019measuring} contains questions paired with SPARQL queries. We use the three MCD splits from the original source.
Similar to previous works
\cite{furrer2020compositional,herzig2021unlocking},
we convert the SPARQL queries into equivalent intermediate representations.

\paragraph{COGS}
The COGS dataset \cite{kim-linzen-2020-cogs} contains sentences paired with logical forms.
We use the generalization test set, which tests generalization to novel linguistic structures.
As SCFG cannot handle logical variables \cite{wong-mooney-2007-learning},
we convert the outputs into equivalent variable-free forms.\tl{What are those variable-free forms? Assure the reader you're not cheating...}
\ice{Give examples for these datasets in the appendix.}\tl{It would be even better to have examples in the paper - just a table with one example of an input + output from each dataset (including the non-synthetic ones) would be great}

\subsubsection{Methods}
Our proposed method, \emph{T5 + CSL-aug}, uses CSL to generate examples for augmenting the training data of T5~\cite{raffel2019exploring}.
For the baselines, we consider T5\footnote{For each dataset, we show results only for the best performing size of T5: T5-Base for SCAN, T5-3B for CFQ, and T5-\textcolor{red}{TODO} for COGS.}
trained on the original training data, T5 trained with additional data generated by GECA~\cite{andreas-2020-good}, and CSL as a standalone parser.
We also report the best published results for each dataset. \ps{More COGS and CFQ baselines to add here: {\tiny\url{http://shortn/_yx6UKZPBPN}}}

\subsubsection{Results and Analysis}

\input{tables/main_synthetic}
\input{tables/main_nonsynthetic}

The results are shown in Table~\ref{tab:main_synthetic}.
For these synthetic datasets, the induced grammars have high coverage, making the CSL model highly effective. When used as a discriminative parser, \fs{the table does not have results on CFQ and COGS}CSL completely solves SCAN and sets new state-of-the-art results on CFQ and COGS.

When we use CSL to generate \fs{Through out, the texts never say how many data is generated.}additional training data for T5, the performance of T5 improves to nearly reaching the accuracy of CSL, demonstrating that we can effectively transfer the compositional generalization ability learned by CSL to T5 via data augmentation.
In addition, compared to GECA, the data produced by CSL gives bigger boosts to T5.

We analyzed the \fs{Where are they?}errors made by T5, CSL, and T5 + CSL-aug. For COGS, T5 struggles at handling recursive modifier phrases, while CSL almost solves such cases.
\ice{Add results from T5 + CSL-aug}
\ice{Add error analysis on CFQ?}

Finally, while an \fs{The result/row is not in the table -- remove this paragraph?}ensemble of CSL and T5 (that favors CSL)\tl{unclear parenthetical. if you want to compare to the ensemble model, describe explicitly earlier} would yield better accuracy than T5 + CSL-aug,
the next section will show that using CSL for data augmentation is better than for model combination in more realistic settings.
% For these synthetic datasets the induced grammars have high coverage, so there is not a need to improve performance on examples that cannot be derived in the induced grammar, which is the main advantage of the data augmentation approach relative to using CSL directly.



\subsection{Non-Synthetic Evaluations}
\label{sec:non-synthetic-evals}

Non-synthetic evaluation of compositional generalization introduces an additional challenge of handling natural language variation. For example, some words in the test data might never appear during training, meaning that a grammar induced from the training data might not derive every input in the test data.
To perform competitively on these benchmarks, we need to leverage information outside the training data, \fs{Not sure what this entails: for the synthetic, we also use T5 pre-trained. So not clear why this is a special point to be made here.}such as by using pre-trained language models.

%In other words, we need to relax our assumptions about the differences between the compositional data generating process for the training and evaluation set. We can still trivially assume that both splits share a common structure, $\mathcal{S}$, but that the subsets of these functions that are used to generate the training and evaluations sets are overlapping but distinct. Alternatively, we can assume some \emph{subset} of the evaluation set can be generated by the same set of functions used to generate the training data. We can measure the effectiveness of our method under such a setting empirically.

\subsubsection{Datasets}
%We compare our methods across various splits of two non-synthetic semantic parsing datasets, GeoQuery and SMCalFlow-CS.

\paragraph{GeoQuery}
The GeoQuery dataset \cite{zelle1996learning} contains human-authored questions paired with meaning representations. We report results on the standard data split as well as three compositional splits introduced in \citet{shaw2021compositional}: the \emph{template} split (where abstract output templates in training and test data are disjoint), the \emph{TMCD} split (an extension of MCD for non-synthetic data), and the \emph{length} split.

\paragraph{SMCalFlow-CS}
\citet{yin2021compositional} proposes a \emph{compositional skill} split of the SMCalFlow dataset \cite{andreas-etal-2020-task} which contains dialog turns paired with meaning representations.
Each training example is a single-turn context-free sentence from one of two domains. The single-domain (S) test set has examples from a single domain, while the cross-domain (C) test set has sentences that require knowledge from both domain. Since compositional language patterns might not be deducible from single-domain training examples, the benchmark has a small amount (8, 16, or 32) of labeled \fs{Is this the same evaluation/training protocol? What if we do not add any samples, ie 0-C?}examples from the test distribution added to the training data.

\subsubsection{Methods}
In addition to the baselines from Section~\ref{sec:synthetic-evals} and best published results,
we also compare our method with \emph{T5 + CSL-ens}, an ensemble model where we use the CSL output if the input has a valid derivation under the induced grammar, and fall back to T5 otherwise. This ensemble approach is similar to NQG-T5 \cite{shaw2021compositional} which performs well on the compositional splits of Geoquery.
\linlu{Can also compare with augmentation with uniform sampling or include this in ablations?}

%For GeoQuery, we compare with NQG-T5 model of ~\citet{shaw2021compositional}, which was shown to be state-of-the-art across the splits evaluated, significantly outperforming todo...

%For SMCalFlow-CS, we compare with the previously reported results from ~\citet{yin2021compositional}.

\paragraph{Semi-supervised learning}
We also evaluate our T5 + CSL-aug model in a setting where some \emph{unlabeled} data from the target distribution is available during training. Concretely, we sample $|\mathcal{U}|$ (128 or 1024) unlabeled inputs from the development set. We then run \fs{Need to make sure this is the same as the "semi-supervised learning" in the previous section.}CSL on these inputs and augment the results to the \fs{Is this also done GeoQuery - I do not thinkt it has more than 1024 to be added?}\linlu{Yes, will probably change this to smaller number}training data.\ice{Is this correct?}

\subsubsection{Results and Analysis}

% \begin{figure}[t]
%     \centering
%    \includegraphics[width=\columnwidth]{figures/quadrant_figures.pdf}
%     \caption{Blah blah blah.}
%     \label{fig:quadrant_figures}
% \end{figure}

As shown in Table~\ref{tab:main_nonsynthetic},
Using CSL to generate additional training data for T5 (T5 + CSL-aug) improves the accuracy of T5 and achieves state-of-the-art on most splits, even when CSL itself under-performs T5. Using CSL for data augmentation is better than using it for model combination (T5 + CSL-ens).

%We also compare results for each split to analyze the relative performance of T5, CSL, and combinations of T5 and CSL using ensembling and data augmentation across inputs that are in-distribution vs. out-of-distribution, and across inputs that can be generated by the induced grammar vs. not. We select the GeoQuery Standard split and the SMCalFlow-CS 16-shot evaluation on single-domain examples for in-distribution evaluations to evaluate, and select the GeoQuery Length split and the SMCalFlow-CS 16-shot evaluation on cross-domain examples as out-of-distrubtion evaluations to analyze. The results are shown in todo... and the aggregated results are plotted in aggregate in Figure~\ref{fig:quadrant_figures}.
To analyze these findings, we compare the models on different types of test inputs.
% As shown in Figure~\ref{fig:quadrant_figures}, we categorize test inputs along two axes:
% (1) whether they are inside the training distribution,\footnote{Results for the in-distribution row come from the GeoQuery standard split and SMCalFlow-CS 16-shot single-domain test set, while results for the out-of-distribution row come from the GeoQuery length split and SMCalFlow-CS  16-shot cross-domain test set.} and (2) whether the they are covered by the induced grammar.
%
CSL can produce outputs only when the input is covered by the grammar (left column), while T5 trained on original training data performs well on in-distribution inputs (bottom row) but struggle at out-of-distribution inputs (top row). While an ensemble model works well on the inputs covered by either CSL or T5, it cannot generalize beyond the base models by definition.

Our data augmentation procedure is akin to \emph{knowledge distillation}. In particular, we distill the ability to compositionally generalize to out-of-distribution inputs (upper left quadrant) from the teacher model CSL to the student model T5.
%We can also see that CSL outperforms T5 on the upper left quadrant of Figure~\ref{fig:quadrant_figures}. This offers an interpretation of our data augmentation procedure as akin to distillation, from the teacher model CSL to the student model T5, where we are primarily interested in \emph{distilling} the relative advantage of CSL on the upper left quadrant to T5.
While many examples generated by CSL would belong to the lower left quadrant (since CSL is trained on in-distribution data),
we will still get examples from the upper left quadrant due to the limited model capacity (such as restricting capacity based on $|\mathcal{T}|$) and conditional independence assumptions (notably, that each rule application in a derivation is conditionally independent of all other rule applications given the parent rule and nonterminal being expanded).

With data augmentation, T5 + CSL-aug gains non-trivial accuracy on the upper right quadrant.
This means that T5 is, to some degree, generalizing from the distillation data (upper and lower left quadrants) to the upper right quadrant.

We finally note that T5 + CSL-aug outperforms T5 + GECA. For a given set of training examples, CSL can derive a significantly larger set of synthetic examples than GECA, We provide some analysis of this in appendix.\ice{TODO!}

==> backup/background_old.tex <==

% \paragraph{What is Compositional Generalization?}
\eat{
The terms compositional, systematic, and combinatorial generalization are often used to refer to the ability to generalize to novel combinations of previously observed ``atoms''. Perhaps the most common example used to illustrate this concept is the human ability to combine words and phrases to produce and understand novel sentences.\cite{fodor1988connectionism} However, despite the intuitive appeal of this description, we often lack a precise description of "atoms" and how they are combined.

Additionally, this ability is commonly assessed by constructing ``out-of-distribution'' evaluations\ps{cite?}. As a guiding principle, it would be helpful to have a clearer theory about what remains the \emph{same} between these training and evaluation distributions.

To address these concerns, we attempt to formulate a more precise problem formulation, appropriate for the semantic parsing and instruction following tasks we study. This problem formulation will also help motivate some aspects of our method.
}
\eat{
$\mathcal{Z}^\mathcal{G}$, 
Let us assume the set of valid inputs is $\mathcal{X}$, and the set of valid outputs is $\mathcal{Y}$. Our data generating process should therefore define a probability distribution over elements $\in \mathcal{X} \times \mathcal{Y}$. First, let us define the \emph{structure} of the data generating process as $\mathcal{S} = \langle \mathcal{F}, \mathcal{X}, \mathcal{Y} \rangle$.

We will define the term \emph{derivation} to mean a ground term $z$ where $\llbracket z \rrbracket \in \mathcal{X} \times \mathcal{Y}$. The set of possible derivations is therefore defined by $\mathcal{S}$, and we will write this set as $\mathcal{Z}^\mathcal{S}$. We will also introduce the following \fs{The $Z^\mathcal{S}$ is $\mathcal{Z}^\mathcal{S}$?  I also changed $y`$ to $y'$ for aesthetics}shorthand notation:
\begin{align*}
\mathcal{Z}^\mathcal{S}_{\langle x,y \rangle} &= \{z \in Z^\mathcal{S} \mid  \llbracket z \rrbracket = \langle x,y \rangle \} \\
\mathcal{Z}^\mathcal{S}_{\langle x,* \rangle} &= \{z \in Z^\mathcal{S} \mid  \exists y'\in\mathcal{Y}, \llbracket z \rrbracket = \langle x,y' \rangle \}
\end{align*}

%$$\mathcal{Z}^\mathcal{S}_{\langle x,y \rangle} = \{z | z \in Z^\mathcal{S} \land \llbracket z \rrbracket = \langle x,y \rangle \}$$

%$$\mathcal{Z}^\mathcal{S}_{\langle x,* \rangle} = \bigcup\limits_{y' \in \mathcal{Y}} \mathcal{Z}^\mathcal{S}_{\langle x,y' \rangle}$$

Given a structure, $\mathcal{S}$, let us assume we have a function, $g$, which assigns probabilities to derivations $z \in \mathcal{Z}^\mathcal{S}$. Given $\mathcal{S}$ and $g$ we can now write the joint probability of our data generating procedure:
$$ p_{\mathcal{S}, g}(x,y) = \sum \limits_{z \in \mathcal{Z}^\mathcal{S}_{\langle x,y \rangle}} g(z).$$
Given this, the conditional distribution is
$$ p_{\mathcal{S}, g}(y|x) = \frac{\sum \limits_{z \in \mathcal{Z}^\mathcal{S}_{\langle x,y \rangle}} g(z)}{\sum \limits_{z \in \mathcal{Z}^\mathcal{S}_{\langle x,* \rangle}} g(z)}.$$

We can now make clear the \fs{Can we say something more such as $P_{\mathcal{S}g_t}(y|x)$ is the same as $P_{\mathcal{S}g_s}(y|x)$ to echo the beginning of the section?}main assumption we will make in this work about the distribution shift between the source and target distributions. We will assume that $p_s(x,y)$ and $p_t(x,y)$ share the same \emph{structure}, $\mathcal{S}$, and that the only difference is the distribution over derivations, which we assume to be different, and which we can refer to as $g_s$ and $g_t$, respectively. Therefore, $p_s(x,y) = p_{\mathcal{S}, g_s}(x,y)$ and $p_t(x,y) = p_{\mathcal{S}, g_t}(x,y)$.\tl{This paragraph is really nice. I wonder if for this paper it wouldn't be enough to zero in on the intuition here. But, as before, you may be conflating "compositional generalization" with "a dataset that diagnoses compositional generalization by creating a shift in the distribution over derivations".}

Of course, such assumptions alone are not sufficient to guarantee the feasibility of compositional generalization. First, $D_{train}$ would need to provide sufficient information to recover, implicitly or explicitly, a sufficient approximation of the underlying structure, $\mathcal{S}$, or a structure isomorphic to it. With no restriction on the class of functions in $\mathcal{F}$, there is seemingly little reason to be optimistic that this is possible in general. Minimally, this requires every function in $\mathcal{S}$ to be observed in $D_{train}$, and some informative prior over structures.\tl{You could give a simple example here---e.g. if an predicate means something different for singular and plural nouns, but the training data only has that predicate appear with singular nouns. But also, not sure this discussion is essential for the paper -- may be good to develop this further in a different paper.}Second, even if we can approximate $g_s$ based on $\mathcal{D}_{train}$, without any \fs{If this is about conditional distribution unchanged across two domains, conditional independence would not be the right term for it.}conditional independence assumptions related to how $g_s$ and $g_t$ decompose over derivations, there could be differences between $g_s$ and $g_t$ that prohibit generalization to new inputs. 

Still, while degenerate cases exist, there are special cases that may suggest some optimism. Recall that our goal is to accurately model $p_t(y|x)$. First, let us consider the case where $|\mathcal{Z}^\mathcal{S}_{\langle x,* \rangle}| = 1$ for all $x \in \mathcal{X}$. In other words, for any given $x$, there is only a single unique derivation in the given structure for $x$. We can therefore see that $p_{\mathcal{S}, g}(y|x)$ \fs{I do not think this is the right way to put it? in this case, $g()$ is defined as $p(x, y)=1$ $y=f(x)$ and 0 otherwise while $f()$ is a deterministic 1-to-1 mapping. So in this case, $p_s$ and $p_g$ are the same.}no longer depends on $g$. Therefore, our ability to model $p_t(y|x)$ is unaffected by any differences between $g_s$ and $g_t$, assuming $\mathcal{S}$ is known, because all probability is assigned to a single $y$. \kt{Does this case mean there is a unique possible y (given by the structure S) for every x? In that case we wouldn't need any probability distribution, but we would just need to return the known y. Seems like this case is not very interesting?}

\eat{
\paragraph{Compositionality and Homomorphisms}

In formal theories about compositionality, a compositional meaning assignment is commonly defined based on a homomorphism between syntactic and semantic structures~\cite{montague1970universal,janssen1997compositionality}. Such ideas have been more recently explored in the context of representation learning by ~\citet{andreas2019measuring} and have inspired recent related work on compositional generalization~\cite{liu2021learning,shaw2021compositional}. We can formally apply this concept of a \emph{compositional mapping} to our setting by placing a restriction on how the functions in $\mathcal{F}$ are formed.

Let us consider two new partial algebras. 
First, let us consider a set of functions $\mathcal{F}^\mathcal{X}$, which generates a set of elements $\mathcal{E}^{\mathcal{F}^\mathcal{X}} \supseteq \mathcal{X}$. Second, let us consider a set of functions $\mathcal{F}^\mathcal{Y}$, which have the same signature as those in $\mathcal{F}^\mathcal{X}$, and which generates a set of elements $\mathcal{E}^{\mathcal{F}^\mathcal{Y}} \supseteq \mathcal{Y}$. We can think of $\mathcal{F}^\mathcal{X}$ as a set of syntactic operators, and $\mathcal{F}^\mathcal{Y}$ as a set of semantic operators, although the outputs for the tasks we study are not necessarily model-theoretic meaning representations.

Now, let us consider a mapping $h : \mathcal{F}^\mathcal{X} \rightarrow \mathcal{F}^\mathcal{Y}$.\footnote{Note that $\mathcal{F}^\mathcal{X}$ can contain multiple equivalent functions which are mapped by $h$ to different functions in $\mathcal{F}^\mathcal{Y}$.}
We can show that this mapping, $h$, defines a homomorphism between the term algebra generated by $\mathcal{F}^\mathcal{X}$ and the algebra generated by $\mathcal{F}^\mathcal{Y}$. We can then form a structure, $\mathcal{S}$, from these two algrebas and $h$, where $\mathcal{E} =  \mathcal{E}^\mathcal{X} \times \mathcal{E}^\mathcal{Y}$ and $\mathcal{F}$ contains a function from $\langle x_1, y_1 \rangle, \cdots, \langle x_k, y_k \rangle$ to $\langle f(x_1, \cdots, x_k), h(f)(y_1, \cdots, y_k) \rangle$ for every $f \in \mathcal{F}^\mathcal{X}$ of arity $k$. If $\mathcal{S}$ is formed in such a way, then we can view $p_{\mathcal{S}, g}(y|x)$ \fs{I would also add ``as defined previously'' or giving an equation number and cite that equation to be clear}as a probabilistic extension of a compositional mapping. \kt{I did not make a connection to how the existence of such a compositional mapping would help us get the train/test generalization right?}

We can interpret Synchronous and Quasi-Synchronous Context Free Grammars (QCFGs), discussed next, together with a probability function $g$, as special cases of such a compositional data generating process. In such formalisms, the class of functions in $\mathcal{F}^\mathcal{X}$ and $\mathcal{F}^\mathcal{Y}$ are essentially limited to string concatenation. The mapping, $h$, is defined by the pairing of rules and linking of nonterminal symbols. QCFGs will be the specific class of structures that we study for the remainder of this paper, although different classes of structures may be more appropriate for other types of tasks.
}
\ps{Removed section on "homomorphisms". Can mention the connection below briefly in QCFG section, and add math to appendix if we want.}

\paragraph{Quasi-Synchronous Context Free Grammars}\ps{copied from ACL paper, need to rewrite.}
\ps{Need to add back connection to $\mathcal{F}$ above.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/derivation_example.pdf}
    \caption{We model the data generating process of each $\langle x,y\rangle$ example as decomposing over a latent \emph{derivation}, as shown above. A set of \emph{functions} can be reused and recombined in novel ways to derive new examples. In this paper we focus on the special case of Quasi-Synchronous Context-Free Grammars (QCFGs). The functions in the derivation above are written as QCFG rules, which generate new string pairs via string concatenation.}
    \label{fig:derivation_example}
\end{figure}

Synchronous Context-Free Grammars (SCFGs) have been used to model the hierarchical mapping between pairs of strings in areas such as compiler theory~\cite{aho1972theory} and natural language processing.\tl{Could add refs to 1990s work here (Smith \& Eisner have some)} Informally,\tl{Why is this informal?} SCFGs can be viewed as an extension of Context-Free Grammars (CFGs) that \emph{synchronously} generate strings in both a source and target language. We write SCFG rules as:
$$ S \rightarrow \langle \alpha,\beta \rangle $$
Where $S$ is a non-terminal symbol, and $\alpha$ and $\beta$ are strings of non-terminal and terminal symbols. An SCFG rule can be viewed as two CFG rules, $S \rightarrow \alpha$ and $S \rightarrow \beta$ with a pairing between the occurrences of non-terminal symbols in $\alpha$ and $\beta$. This pairing is indicated by assigning each non-terminal in $\alpha$ and $\beta$ an index $\in \mathbb{N}$. Non-terminals sharing the same index are called \emph{linked}. Following convention, we denote the index for a non-terminal using a boxed subscript, e.g. $NT_{\boxnum{1}}$. A complete SCFG derivation is a pair of parse trees, one for the source language and one for the target language. An example derivation is shown in Figure ~\ref{fig:derivation_example}.

Quasi-Synchronous Context Free Grammars (QCFGs) generalize SCFGs in various ways,\tl{it would be good to say a little bit about those ways} notably relaxing the restriction on a \fs{Come to think about this a bit:  if the language of SMM, this means $h$ is what kind of function?}strict one-to-one alignment between source and target non-terminals~\cite{smith2006quasi}. 
}

==> backup/csl_vs_geca.tex <==
\begin{table}[!ht]
\begin{center}
\scalebox{0.59}{
\begin{tabular}{lll}
\toprule
\normalsize
& \multicolumn{1}{c}{GECA} & \multicolumn{1}{c}{CSL} \\
\midrule
\multirow{3}{*}{{\begin{tabular}[c]{@{}l@{}}Training \\ Examples \end{tabular}}} &  \multicolumn{2}{l}{$\langle$jump, JUMP$\rangle$} \\
& \multicolumn{2}{l}{$\langle$walk, WALK$\rangle$} \\ 
& \multicolumn{2}{l}{$\langle$jump and walk, JUMP WALK$\rangle$} \\ 
% \midrule
% \multirow{2}{*}{{\begin{tabular}[c]{@{}l@{}}Induced \\ Rules \end{tabular}}} & \multicolumn{2}{l}{$\mbox{NT} \rightarrow \langle \mbox{NT}_\boxnum{1}$ $\mbox{NT}_\boxnum{2},~\mbox{NT}_\boxnum{1}~ \mbox{NT}_\boxnum{2} \rangle$} \\ 
% & \multicolumn{2}{l}{$\mbox{NT} \rightarrow \langle$walk, WALK$\rangle$, $\mbox{NT} \rightarrow \langle$jump, JUMP$\rangle$} \\ 
\midrule
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Derivable \\ Examples\end{tabular}} & \multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}$\langle$walk and walk, WALK WALK$\rangle$ \\ $\langle$jump and jump, JUMP JUMP$\rangle$ \end{tabular}} & $\langle$walk and walk, WALK WALK$\rangle$ \\
 &  & $\langle$jump and jump, JUMP JUMP$\rangle$ \\
& & $\langle$walk and jump, WALK JUMP$\rangle$ \\
& & $\langle$walk and walk and jump, \\
& & WALK WALK JUMP$\rangle$ \\
& & $\langle$walk and jump and walk and walk, \\
& & WALK JUMP WALK WALK$\rangle$ \\
& & ... \\
\bottomrule
\end{tabular}
}
\caption{We show the set of derivable synthetic examples for GECA and CSL, given an illustrative example of training examples. CSL can derive a significantly larger set of synthetic examples than GECA, and also assigns a probability to each derivable example.} 
\label{tab:csl_vs_geca}
\end{center}
\end{table}


==> backup/csl_vs_geca_old.tex <==

\begin{table}[!ht]
\begin{center}
\scalebox{0.82}{
\begin{tabular}{l}
\toprule
Given training examples:\\
\\
$\langle foo , bar \rangle$ \\
$\langle foo , bar \rangle$ \\
$\cdots$ \\
\midrule
Induce a generative model with latent rules:\\
\\
$NT \rightarrow \langle foo , bar \rangle$ \\
$NT \rightarrow \langle foo , bar \rangle$ \\
$\cdots$ \\
\midrule 
Sample new synthetic examples from generative model:\\
\\
$\langle foo , bar \rangle$ \\
$\langle foo , bar \rangle$ \\
$\cdots$ \\
\sout{$\langle foo , bar \rangle$} \\
\bottomrule
\end{tabular}
}
\caption{TODO... write this and improve figure... CSL uses an iterative optimization algorithm to select from a less restricted set of grammars, enabling a larger set of synthetic examples expressing recombinations of the original training data than prior work. Additionally, CSL learns a probabilistic generative model, so it can assign low probability to low quality synthetic examples that could otherwise be generated by the induced grammar (illustrated with \sout{strikethough}). } 
\label{tab:csl_vs_geca}
\end{center}
\end{table}

\linlu{Will this be a good example? training examples, "jump and run after walk", "jump", "run", "walk", GECA won't synthesize anything. But CSL can learn "NT -> NT1 and NT2 after NT3" which provides many combinations}

==> backup/method_diagram_v2.tex <==
\newcommand{\lispress}[1]{{\fontfamily{cmtt}\selectfont #1}}
\newcommand{\ddone}[1]{{\textcolor{dgreen}{#1}}}
\newcommand{\ddtwo}[1]{{\textcolor{dblue}{#1}}}
\newcommand{\ddthree}[1]{{\textcolor{dred}{#1}}}
\newcommand{\ddfour}[1]{{\textcolor{dyellow}{#1}}}

\renewcommand{\ddone}[1]{\colorbox{orange!10!white}{#1}}
\renewcommand{\ddtwo}[1]{\colorbox{red!8!white}{#1}}
\renewcommand{\ddthree}[1]{\colorbox{blue!8!white}{#1}}
\renewcommand{\ddfour}[1]{\colorbox{dgreen!10!white}{#1}}

\begin{figure}[!t]
\begin{center}

\scalebox{0.7}{


\begin{tikzpicture} % [node distance=0.5cm]
\begin{scope}[every node/.style={inner xsep=5pt, inner ysep=5pt}]

\tikzstyle{examples} = [rectangle, draw=black, fill=none, inner ysep=1.8ex]

\tikzstyle{process} = [rectangle, rounded corners, text centered, draw=black, fill=cellshade,inner xsep=6pt, inner ysep=4pt]
\tikzstyle{model} = [rectangle, text centered, draw=dblue, fill=lblue,inner xsep=7pt, inner ysep=7pt]

\tikzstyle{arrow} = [thick,->,>=latex]

\node (n1) [examples, text width=10.5cm] {
%
{\centering{\textbf{\textsc{Original Examples}}}\\[1ex]}
%
\textit{Add an event for {\ddone{next Tuesday}} to my calendar} \\
$\to$ \lispress{(CreateEvent {\ddone{:start (NextDOW :dow TUE)}})} \\

\textit{{\ddtwo{Create a meeting with}}{\ddthree{Alice\vphantom{g}}}} \\
$\to$ \lispress{{\ddtwo{(CreateEvent :attendees}}{\ddthree{(Contact :name "Alice")}}{\ddtwo{)}}} \\
\textit{Who is on Bob{\ddfour{'s team}}} \\
$\to$ \lispress{{\ddfour{(FindTeamOf :recipient}}(Contact :name "Bob"){\ddfour{)}}} \hfill \dots
};

\node (n2) [process, below=0.3cm of n1, align=center] {Train CSL, a generative model with latent compositional structure};

\node (n3) [model, below=0.3cm of n2, align=center] {CSL};

\node (n4) [process, below=0.3cm of n3, align=center] {Sample synthetic examples from CSL};

\node (n5) [examples, text width=10.5cm, below=0.3cm of n4]{
%
{\centering{\textbf{\textsc{Synthetic Examples}}}\\[1ex]}
% The \vphantom{g} is to make the boxes fill the vertical space
\textit{{\ddtwo{Create a meeting with}}{\ddthree{Alice\vphantom{g}}}{\ddfour{'s team\vphantom{g}}}{\ddone{next Tuesday}}} \\
$\to$ \lispress{{\ddtwo{(CreateEvent :attendees}}{\ddfour{(FindTeamOf :recipient}} \\
{\ddthree{(Contact :name "Alice")}}{\ddfour{)}}{\ddone{:start (NextDOW :dow TUE)}}{\ddtwo{)}}}
};

\node (n6) [process, below=0.3cm of n5, align=center] {Train T5 on original and synthetic examples};

\node (n7) [model, below=0.3cm of n6, align=center] {Augmented T5};

\draw [arrow] (n1) -- (n2);
\draw [arrow] (n2) -- (n3);
\draw [arrow] (n3) -- (n4);
\draw [arrow] (n4) -- (n5);
\draw [arrow] (n5) -- (n6);
\draw [arrow] (n6) -- (n7);

\end{scope}
\end{tikzpicture}

}

\end{center}

\caption{
An overview of our method for compositional data augmentation with CSL, a generative model with a QCFG backbone, which is automatically induced from the training data. We show a notional set of original and synthetic examples mapping utterances to programs.
}
\label{fig:method_diagram}
\end{figure}


==> backup/method_diagram_v2_old.tex <==

\begin{figure}[!t]
\begin{center}

\scalebox{0.7}{


\begin{tikzpicture} % [node distance=0.5cm]
\begin{scope}[every node/.style={inner xsep=5pt, inner ysep=5pt}]

\tikzstyle{examples} = [rectangle, draw=black, fill=none]
% \tikzstyle{process} = [rectangle, text centered, draw=none, fill=none]
\tikzstyle{process} = [rectangle, rounded corners, text centered, draw=black, fill=cellshade,inner xsep=6pt, inner ysep=4pt]
\tikzstyle{model} = [rectangle, text centered, draw=dblue, fill=lblue,inner xsep=7pt, inner ysep=7pt]

\tikzstyle{arrow} = [thick,->,>=latex]

\node (n1) [examples,  text width=7.5cm] {

{\centering{\textsc{Original Examples}}\\[0.2cm]}

\textit{Add an event for {\textcolor{dyellow}{next Tuesday}} to my calendar} \\
\textit{{\textcolor{dblue}{Create a meeting with}} {\textcolor{dred}{Alice}} at 3pm } \\
\textit{Who is on Bob{\textcolor{dgreen}{'s team}}} \\
$\cdots$
};

\node (n2) [process, below=0.3cm of n1, align=center] {Train CSL, a generative model with latent compositional structure};

\node (n3) [model, below=0.3cm of n2, align=center] {CSL};

\node (n4) [process, below=0.3cm of n3, align=center] {Sample synthetic examples from CSL};

\node (n5) [examples, text width=8.5cm, below=0.3cm of n4]{

{\centering{\textsc{Synthetic Examples}}\\[0.2cm]}

\textit{{\textcolor{dblue}{Create a meeting with}} {\textcolor{dred}{Alice}}{\textcolor{dgreen}{'s team}} {\textcolor{dyellow}{next Tuesday}}} \\
$\cdots$
};

\node (n6) [process, below=0.3cm of n5, align=center] {Train T5 on original and synthetic examples};

\node (n7) [model, below=0.3cm of n6, align=center] {Augmented T5};

\draw [arrow] (n1) -- (n2);
\draw [arrow] (n2) -- (n3);
\draw [arrow] (n3) -- (n4);
\draw [arrow] (n4) -- (n5);
\draw [arrow] (n5) -- (n6);
\draw [arrow] (n6) -- (n7);

\end{scope}
\end{tikzpicture}

}

\end{center}

\caption{
An overview of our method for compositional data augmentation with CSL, a generative model with a QCFG backbone, which is automatically induced from the training data. We show a notional set of original and synthetic examples.
}
\label{fig:method_diagram}
\end{figure}



\eat{

$\langle$ The girl ate the cake on the table, \\ eat(agent=*girl, theme=cake(nmod.on=*table) $\rangle$ \\[0.2cm]

$\langle$ Jack saw a dog in the house, \\
see(agent=Jack, theme=dog(nmod.in=*house)) $\rangle$ \\[0.2cm]

$\langle$ The dog saw a cake on the table in the house, \\
see(agent=*dog,theme=*cake(nmod.on=*table(nmod.in=*house))) $\rangle$ \\[0.2cm]

}

==> backup/semisupervised.tex <==
\begin{table}[!t]
\begin{center}

\scalebox{0.82}{
\begin{tabular}{lcccccc}
\toprule
Setting & 8-S & 8-C & 16-S & 16-C & 32-S & 32-C \\
\midrule
Sup. & 
81.7 & 51.0 & 81.0 & 63.1 & 81.9 & 67.34 \\
Semi-sup. & 
--- & --- & --- & --- & --- & --- \\
\bottomrule
\end{tabular}
}
\caption{Accuracy of T5+CSL-Aug. for SMCalFlow-CS using the standard supervised learning setting comapred with the semi-supervised learning setting where we allow the model to use unlabeled inputs from the dev set.)
} 
\label{tab:semisupervised}
\end{center}
\end{table}



